Robust massive MIMO Equilization for mmWave systems with low resolution ADCs

Leveraging the available millimeter wave spectrum will be important for 5G. In this work, we investigate the performance of digital beamforming with low resolution ADCs based on link level simulations including channel estimation, MIMO equalization and channel decoding. We consider the recently agreed 3GPP NR type 1 OFDM reference signals. The comparison shows sequential DCD outperforms MMSE-based MIMO equalization both in terms of detection performance and complexity. We also show that the DCD based algorithm is more robust to channel estimation errors. In contrast to the common believe we also show that the complexity of MMSE equalization for a massive MIMO system is not dominated by the matrix inversion but by the computation of the Gram matrix.

==> Introduction/pics/OverviewModelpsfrag.tex <==
%% Creator: Inkscape inkscape 0.92.0, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'OverviewModelpsfrag.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{456.27998859bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.29313141)%
    \put(0,0){\includegraphics[width=\unitlength]{./Introduction/pics/OverviewModelpsfrag.eps}}%
    \put(0.30621548,0.15237354){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{multipath}}}%
    \put(0.31417112,0.12590953){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{channel}}}%
    \put(0.56211098,0.04432585){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_C$}}}%
    \put(0.56211098,0.19916499){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_C$}}}%
    \put(0.09391163,0.19916499){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_T$}}}%
    \put(0.09391163,0.04432585){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_T$}}}%
    \put(0.07632375,0.12174542){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M$}}}%
    \put(0.01594416,0.19916499){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{UE $1$}}}%
    \put(0.01594416,0.04432585){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{UE $M$}}}%
    \put(0.81824757,0.12174542){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_{\text{RFE}}$}}}%
    \put(0.92224073,0.13500482){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{digital}}}%
    \put(0.9094854,0.10854081){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{baseband}}}%
    \put(0.79409573,0.21242439){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{A/D}}}%
    \put(0.76483738,0.18596038){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{conversion}}}%
    \put(0.64701499,0.07078987){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{analog}}}%
    \put(0.65003945,0.04432585){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{signal }}}%
    \put(0.62137284,0.01791663){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{combination}}}%
    \put(0.79409573,0.05758525){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{A/D}}}%
    \put(0.76483738,0.03112124){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{conversion}}}%
    \put(0.64701499,0.225629){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{analog}}}%
    \put(0.65003945,0.19916499){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{signal}}}%
    \put(0.62137284,0.17275576){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{combination}}}%
  \end{picture}%
\endgroup%


==> SignalModel/pics/CS_orthogonality.tex <==
%% Creator: Inkscape inkscape 0.92.0, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'CS_orthogonality.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{204.30502418bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.50738964)%
    \put(0,0){\includegraphics[width=\unitlength]{./SignalModel/pics/CS_orthogonality.eps}}%
    \put(-0.00095431,0.00054945){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{time}}}%
    \put(0.11933152,0.31331708){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{CP}}}%
  \end{picture}%
\endgroup%


==> SignalModel/pics/SignalModel_1col.tex <==
%% Creator: Inkscape 0.91_64bit, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'SignalModel_1col.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{230.61bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.3953211)%
    \put(0,0){\includegraphics[width=\unitlength]{./SignalModel/pics/SignalModel_1col.eps}}%
    \put(0.70420493,0.19273349){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$F(\cdot)$}}}%
    \put(0.90066693,0.19273349){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{r}[n]$}}}%
    \put(0.43429513,0.02066332){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{\eta}[n]$}}}%
    \put(0.57036902,0.24780482){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{y}[n]$}}}%
    \put(0.51278262,0.10413759){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_R$}}}%
    \put(0.01087941,0.29062603){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1[n]$}}}%
    \put(0.01087941,0.09126347){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_M[n]$}}}%
    \put(0.21088817,0.29062603){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{h}_1$}}}%
    \put(0.21088817,0.09375686){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{h}_M$}}}%
  \end{picture}%
\endgroup%


==> SignalModel/pics/SignalModel_2col.tex <==
%% Creator: Inkscape 0.91_64bit, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'SignalModel_2col.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{203.55bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.39532793)%
    \put(0,0){\includegraphics[width=\unitlength]{./SignalModel/pics/SignalModel_2col.eps}}%
    \put(0.70702284,0.19334144){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$F(\cdot)$}}}%
    \put(0.90336527,0.19334144){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{r}[n]$}}}%
    \put(0.43687055,0.02197347){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{\eta}[n]$}}}%
    \put(0.57307787,0.2484876){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{y}[n]$}}}%
    \put(0.51397691,0.11461385){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$M_R$}}}%
    \put(0.02112503,0.29135176){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1[n]$}}}%
    \put(0.02112503,0.09422574){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_M[n]$}}}%
    \put(0.21432081,0.29135176){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{h}_1$}}}%
    \put(0.21432081,0.09422574){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\boldsymbol{h}_M$}}}%
  \end{picture}%
\endgroup%

